Measuring NUMA effects with the STREAM benchmark

Modern high-end machines feature multiple processor packages, each of which contains multiple independent cores and integrated memory controllers connected directly to dedicated physical RAM. These packages are connected via a shared bus, creating a system with a heterogeneous memory hierarchy. Since this shared bus has less bandwidth than the sum of the links to memory, aggregate memory bandwidth is higher when parallel threads all access memory local to their processor package than when they access memory attached to a remote package. But, the impact of this heterogeneous memory architecture is not easily understood from vendor benchmarks. Even where these measurements are available, they provide only best-case memory throughput. This work presents a series of modifications to the well-known STREAM benchmark to measure the effects of NUMA on both a 48-core AMD Opteron machine and a 32-core Intel Xeon machine.

==> common/lstlang-bomil.tex <==
\lstdefinelanguage{BOMIL}{%
  morekeywords={%
    addr, alloc, and, any, apply, bool, byte, case, ccall, cont, define, do, double,%
    enum, extern, false, float, fun, host_vproc, if, inline, int, let, long, module,%
    noreturn, promote, pure, return, short, tag, throw, true, typedef, unwrap, use_rw,%
    vec128, void, vproc, vpload, vpstore, wrap,%
  },%
  keywordsprefix=@,
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> common/lstlang-manticore.tex <==
\lstdefinelanguage{Manticore}[]{SML}{%
  morekeywords={by,otherwise,pcase,pval,spawn,to},
  % otherkeywords={(|,|),[|,|],(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  otherkeywords={(|,|),[|,|],?,\&},
}[keywords,comments,strings]%


==> common/lstlang-sml.tex <==
\lstdefinelanguage{SML}{%
  morekeywords={%
    abstype, and, andalso, as, case, datatype, do, else, end, eqtype, exception,%
    fn, fun, functor, handle, if, in, include, infix, infixr, let, local, nonfix,%
    of, op, open, orelse, raise, rec, sharing, sig, signature, struct, structure,%
    then, type, val, where, while, with, withtype,%
  },%
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> common/slide-defs.tex <==
% slide-defs.tex
%
% common definitions for talks.
%
% define \TalkDate and \TalkTitle for footers
%

% for a 1024x768 screen, we have a 1.0:0.75 ratio.
\setlength{\textwidth}{9.3in}
\setlength{\textheight}{7.2in}
\addtolength{\leftmargin}{-0.15in}
\addtolength{\topmargin}{-0.7in}

\usepackage{color}
\usepackage{graphicx}
\usepackage{times}

%
% the following magic makes the tt font in math mode be the same as the
% normal tt font (i.e., Courier)
%
\SetMathAlphabet{\mathtt}{normal}{OT1}{pcr}{n}{n}
\SetMathAlphabet{\mathtt}{bold}{OT1}{pcr}{bx}{n}

\definecolor{Red}{rgb}{0.8,0.0,0.0}
\definecolor{Green}{rgb}{0.0,0.4,0.0}
\definecolor{Blue}{rgb}{0.0,0.0,0.9}
\definecolor{Purple}{rgb}{0.5,0.0,0.4}
\definecolor{Black}{rgb}{0.0,0.0,0.0}
\definecolor{Yellow}{rgb}{1.0,1.0, 0.25}
\definecolor{Cyan}{rgb}{0.25,1.0, 1.0}
\newcommand{\blue}[1]{\color{Blue}{#1}}
\newcommand{\red}[1]{\color{Red}{#1}}
\newcommand{\green}[1]{\color{Green}{#1}}
\newcommand{\purple}[1]{\color{Purple}{#1}}
\newcommand{\textblue}[1]{\textcolor{Blue}{#1}}
\newcommand{\textred}[1]{\textcolor{Red}{#1}}
\newcommand{\textgreen}[1]{\textcolor{Green}{#1}}
\newcommand{\textpurple}[1]{\textcolor{Purple}{#1}}
\newcommand{\textblack}[1]{\textcolor{Black}{#1}}

\newcommand{\mobycodecolor}{\color{Purple}}
\newcommand{\punctcolor}{\color{Blue}}
\newcommand{\kwcolor}{\color{Blue}}
\newcommand{\bolcodecolor}{\color{Green}}
\newcommand{\ccodecolor}{\color{Purple}}
%\newcommand{\highlightC}[1]{\textred{#1}}
\newcommand{\highlightC}[1]{\colorbox{Yellow}{#1}}
\newcommand{\highlightCC}[1]{\colorbox{Cyan}{#1}}

\newcommand{\BlueBullet}{\textcolor{Blue}{\ensuremath{\bullet}}}
\newcommand{\RedBullet}{\textcolor{Red}{\ensuremath{\bullet}}}
\newcommand{\GreenBullet}{\textcolor{Green}{\ensuremath{\bullet}}}

\newcommand{\EM}[1]{\emph{\textred{#1}}}

\raggedright
\pagestyle{empty}

\newcommand{\HEAD}[1]{
  \noindent{\large\bf{}#1}\\[-1ex]
  \textblue{\hrulefill}\\[1em]}
\newcommand{\CONTINUE}[1]{
  \noindent{\bf{}#1 {\it{}(continued ...)}}\\[-1ex]
   \textblue{\hrulefill}\\[1em]}
\newcommand{\CHEAD}[1]{{\makebox[\textwidth]{\large\bf{}#1}\\[1em]}}
\newcommand{\FOOT}{%
  \vfill\textblue{\hrulefill}\\ %
  \tiny{
    \mbox{\rule[-.5ex]{0em}{3ex}} %
    \TalkDate  \hfill \TalkTitle \hfill \arabic{slide}}%
}

\newenvironment{FIGURE}{%
  \begin{center}\small}{%
  \end{center}}

% code
\newcommand{\tkw}[1]{\text{\kw{#1}}}
\newcommand{\tcd}[1]{\text{\cd{#1}}}
 

==> evaluation.tex <==
%!TEX root = paper.tex

\section{Evaluation}
\label{sec:evaluation}
Our AMD test machine is described in \secref{intro:amdhardware}.
This machine runs x86\_64 Ubuntu Linux 10.04.2 LTS, kernel version 2.6.32-27.
\secref{intro:intelhardware} describes our Intel test machine.
This machine runs x86\_64 RedHat Enterprise Linux, kernel version
2.6.18-194.11.4.el5.
The \vproc{} local heap size is 1~MB, which is slightly more than the L3~cache
size when nodes each have 6~threads.
We ran each experiment 10 times and we report the average performance results in
our graphs and tables.

\subsection{Benchmarks}
For our empirical evaluation, we use five benchmark programs from our benchmark suite
and one synthetic benchmark.
Each benchmark is written in a pure, functional style and was originally written
by other researchers and ported to our system.

The Barnes-Hut benchmark~\cite{barnes-hut} is a classic N-body problem solver.
Each iteration has two phases.
In the first phase, a quadtree is constructed from a sequence of mass points.
The second phase then uses this tree to accelerate the computation of
the gravitational force on the bodies in the system.
Our benchmark runs 20 iterations over 400,000 particles generated in
a random Plummer distribution.
Our version is a translation of a Haskell
program~\cite{barnes-hut-haskell-bench}. 

The Raytracer benchmark renders a $512 \times 512$ image in parallel as
two-dimensional sequence, which is then written to a file.
The original program was written in ID~\cite{id90-manual} and is a simple
ray tracer that does not use any acceleration data structures.
The sequential version differs from the parallel code in that it
outputs each pixel to the image file as it is computed, instead of building
an intermediate data structure.

The Quicksort benchmark sorts a sequence of 10,000,000 integers in parallel.
This code is based on the \nesl{} version of the algorithm~\cite{scandal-algorithms}.

The SMVM benchmark is a sparse-matrix by dense-vector multiplication.
The matrix contains 1,091,362 elements and the vector 16,614.

The DMM benchmark is a dense-matrix by dense-matrix multiplication in which
each matrix is $600 \times 600$.

\begin{figure*}
\vspace*{-0.5in}
\begin{center}
AMD Speedups\\
  \includegraphics[width=6in]{data/results/amd/speedup} \\[3em]
Intel Speedups\\
  \includegraphics[width=6in]{data/results/intel/speedup} \\
\end{center}%
\caption{ 
  Comparative speedup plots for five benchmarks on both AMD and Intel hardware.
  The baseline is the single-processor version of each benchmark.
  Larger speedup values are better, and speedup values equal to the number of
  threads are ideal.
}
\label{fig:speedups} 
\end{figure*}%

\subsection{Performance}
The dense-matrix multiplication (DMM) and raytracer benchmarks have abundant,
independent parallelism and our compiler and runtime exploit them, demonstrating
nearly ideal speedup up to the maximum number of cores on both machines.
Quicksort, sparse-matrix multiplication, and barnes-hut have excellent behavior
until either 24~or 36~threads, but then taper off.

On the AMD machine, both quicksort and barnes-hut scale nicely to 36~threads but
then only take slight advantage of additional threads.
In barnes-hut, we believe that this behavior is due to the sequential portion.
Quicksort also is limited by its fork-join parallelism, and without
significantly increasing the size of the underlying dataset, it is difficult to
take advantage of the additional available parallelism.

Sparse-matrix multiplication provides the least scalability for the AMD system.
We believe that this is due to a large amount of available execution parallelism
but a relatively small amount of data.
Unless this data is either perfectly divided between the nodes or replicated to
each location, this benchmark fails to take much advantage of greater than even
24~threads.

On the Intel machine, quicksort, barnes-hut, and spare-matrix multiplication
(SMVM) all see reducing speedups past 16~threads, but do not experience the more
serious lack of speedups seen on the AMD machine.
We believe that this better performance, particularly on SMVM, is due to a
smaller NUMA penalty when accessing the relatively smaller amount of shared
data, much of which resides on only one node.
Additionally, with only 4~nodes on the Intel machine, threads are twice as
likely to be located near data even if that data was placed randomly.

\paragraph{Locality affects scalability}
As these benchmarks and the figures in \secref{sec:numa} have shown, locality
and NUMA effects have an impact on benchmarks.
Benchmarks such as dense-matrix multiplication and raytracer, with excellent
locality and almost no shared data can scale nearly perfectly if all of their
data is kept locally.
The other benchmarks, which feature either heavily shared data or significant
points that sequentially merge data before creating more parallel work show
diminished improvements.
Unfortunately, these effects do not even easily show up on machines with
multiple processor packages until relatively large numbers of cores --- in our
experience, between 24~and~36.
Further, testing a runtime on a machine with a large number of cores but where
all are on the same processor package provides no feedback on the NUMA
scalability of that runtime.

\subsection{Load-balanced global collections}
\label{sec:evalGlobal}
During our global copying heap collection, there is often imbalanced available
work.
This imbalance results from uneven allocation patterns by threads,\footnote{In
  particular, when a large data file is sequentially read into memory.} and
causes there to be extra blocks of to-space available to scan.
Prior work on the Glasgow Haskell Compiler (GHC) showed increased times when
parallel collections also performed global load-balancing of this imbalanced
work~\cite{multicore-haskell}.
As we show in \tblref{eval:load-balanced}, load-balancing is very effective when
performed on a per-node basis.
We compare the performance of a unbalanced collections with balanced
collections on our AMD machine, where in the latter case threads will scan
unscanned chunks generated from any thread, so long as it is on the same node.
Execution times are measured in seconds, and lower numbers are better.
The DMM, SMVM, and raytracer benchmarks are not included because none of those
programs keep data around for long enough to trigger a global GC collection.
Barnes-hut and quicksort both see greater than a 15\% reduction in global GC
time and a nearly 3\% reduction in overall execution time, when run on
48~cores.
\begin{table}
  \begin{center}
  \begin{tabular}{r | c | c | c | c}
 & \multicolumn{2}{c|}{Unbalanced} & \multicolumn{2}{c}{Balanced} \\
Benchmark & Global (s) & Total (s) & Global (s) & Total (s)\\
\hline
Barnes-hut & 0.308 & 2.52 & 0.255 & 2.45 \\
Quicksort & 0.321 & 2.16 & 0.268 & 2.10 \\
% Barnes-hut & 82.8\% & 97.2\% \\
% Quicksort & 83.5\% & 97.2\% \\
\end{tabular}
\end{center}
\caption{
  Comparison of load-balanced versus unbalanced global collections on 48
  cores on the AMD machine. Smaller numbers are better.
}
\label{eval:load-balanced}
\end{table}%

\subsection{Single-thread performance versus a sequential program}

As is shown in \tblref{eval:mlton}, only on the raytracer do we offer
competitive performance to the sequential MLton baseline.
On all other benchmarks, we generally reach speed parity with four threads on
the AMD machine.
This performance gap is due to missed opportunities for sequential optimization
in Manticore and some small overhead from our parallel language constructs.
But, given that MLton has state-of-the-art functional language performance, this
comparison demonstrates that we have performance comparable with mainstream
functional languages on these benchmarks.

\begin{table}
  \begin{center}
  \begin{tabular}{r | c | c | c | c}
Benchmark & MLton (s) & 1T (s) & 2T (s) & 4T (s)\\
\hline
Barnes-hut & 20.4 & 61.4 & 38.2 & 17.0 \\
DMM & 12.4 & 50.6 & 27.6 & 12.6 \\
Quicksort & 20.9 & 100.8 & 52.5 & 27.5 \\
Raytracer & 10.9 & 15.6 & 7.7 & 3.9 \\
SMVM & 7.2  & 28.3 & 15.0 & 7.6\\
\end{tabular}
\end{center}
\caption{
  Comparison of Manticore performance versus MLton at low numbers of
  threads on the AMD machine. Smaller execution times are better.
}
\label{eval:mlton}
\end{table}%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

